Weak-Instrument Inference and Model Diagnostics in Double Machine Learning for Linear Instrumental Variable Models

We study weak-instrument-robust inference in partially linear instrumental-variables models with learned nuisances. Building on an i.i.d. uniform-size baseline, we establish uniform asymptotic validity of clustered cross-fitted Anderson-Rubin inference and cross-fitted score inference under the stated sampling and nuisance-rate conditions. Extensions establish Anderson-Rubin validity for survey-weighted target laws and fold-nested generated instruments. A supporting population benchmark shows that prediction-optimal instrument residualization maximizes concentration when the treatment nuisance is correctly specified. A five-design diagnostic portfolio, a known-truth Monte Carlo, and an exploratory selector examine how nuisance specification and estimation affect realized strength and inference.

==> supplementary_numbers.tex <==
\makeatletter
\expandafter\gdef\csname r@a.1-proposition-1-sources-and-proof-sketch\endcsname{{A.1}{}{}{}{}}
\expandafter\gdef\csname r@a.2-proposition-2-weak-identification-limit\endcsname{{A.2}{}{}{}{}}
\expandafter\gdef\csname r@a.3-proof-of-proposition-3\endcsname{{A.3}{}{}{}{}}
\expandafter\gdef\csname r@a.4-proof-of-theorem-1\endcsname{{A.4}{}{}{}{}}
\expandafter\gdef\csname r@a.5-proof-of-theorem-2\endcsname{{A.5}{}{}{}{}}
\expandafter\gdef\csname r@a.6-weighted-and-generated-instrument-extensions\endcsname{{A.6}{}{}{}{}}
\expandafter\gdef\csname r@app:c\endcsname{{C}{}{}{}{}}
\expandafter\gdef\csname r@app:d\endcsname{{D}{}{}{}{}}
\expandafter\gdef\csname r@app:d1\endcsname{{D.1}{}{}{}{}}
\expandafter\gdef\csname r@app:d2\endcsname{{D.2}{}{}{}{}}
\expandafter\gdef\csname r@app:d4\endcsname{{D.4}{}{}{}{}}
\expandafter\gdef\csname r@app:d5\endcsname{{D.5}{}{}{}{}}
\expandafter\gdef\csname r@app:d6\endcsname{{D.6}{}{}{}{}}
\expandafter\gdef\csname r@app:e\endcsname{{E}{}{}{}{}}
\expandafter\gdef\csname r@app:f\endcsname{{F}{}{}{}{}}
\expandafter\gdef\csname r@appendix-a-formal-results-sources-and-proofs\endcsname{{A}{}{}{}{}}
\expandafter\gdef\csname r@c.5-set-extraction\endcsname{{C.5}{}{}{}{}}
\expandafter\gdef\csname r@lem:cfjoint\endcsname{{1}{}{}{}{}}
\expandafter\gdef\csname r@lem:within-bridge\endcsname{{9}{}{}{}{}}
\expandafter\gdef\csname r@prop:generated\endcsname{{5}{}{}{}{}}
\expandafter\gdef\csname r@prop:weighted\endcsname{{4}{}{}{}{}}
\expandafter\gdef\csname r@tab:1\endcsname{{D.1}{}{}{}{}}
\expandafter\gdef\csname r@tab:2\endcsname{{D.2}{}{}{}{}}
\expandafter\gdef\csname r@tab:b1\endcsname{{B.1}{}{}{}{}}
\expandafter\gdef\csname r@tab:b10\endcsname{{B.10}{}{}{}{}}
\expandafter\gdef\csname r@tab:b11\endcsname{{B.11}{}{}{}{}}
\expandafter\gdef\csname r@tab:b12\endcsname{{B.12}{}{}{}{}}
\expandafter\gdef\csname r@tab:b2\endcsname{{B.2}{}{}{}{}}
\expandafter\gdef\csname r@tab:b3\endcsname{{B.3}{}{}{}{}}
\expandafter\gdef\csname r@tab:b4\endcsname{{B.4}{}{}{}{}}
\expandafter\gdef\csname r@tab:b5\endcsname{{B.5}{}{}{}{}}
\expandafter\gdef\csname r@tab:b6\endcsname{{B.6}{}{}{}{}}
\expandafter\gdef\csname r@tab:b7\endcsname{{B.7}{}{}{}{}}
\expandafter\gdef\csname r@tab:b9\endcsname{{B.9}{}{}{}{}}
\expandafter\gdef\csname r@thm:iid-import\endcsname{{A.1}{}{}{}{}}
\makeatother

